Recurrent CircuitSAT Sampling for Sequential Circuits

In this work, we introduce a novel GPU-accelerated circuit satisfiability (CircuitSAT) sampling technique for sequential circuits. This work is motivated by the requirement in constrained random verification (CRV) to generate input stimuli to validate the functionality of digital hardware circuits. A major challenge in CRV is generating inputs for sequential circuits, along with the appropriate number of clock cycles required to meet design constraints. Traditional approaches often use Boolean satisfiability (SAT) samplers to generate inputs by unrolling state transitions over a fixed number of clock cycles. However, these methods do not guarantee that a solution exists for the given number of cycles. Consequently, producing input stimuli together with the required clock cycles is essential for thorough testing and verification. Our approach converts the logical constraints and temporal behavior of sequential circuits into a recurrent CircuitSAT problem, optimized via gradient descent to efficiently explore a diverse set of valid solutions, including their associated number of clock cycles. By operating directly on the circuit structure, our method reinterprets the sampling process as a supervised multi-output regression task. This differentiable framework enables independent element-wise operations on each tensor element, facilitating parallel execution during learning. As a result, we achieve GPU-accelerated sampling with substantial runtime improvements (up to 105.1x) over state-of-the-art heuristic samplers. We demonstrate the effectiveness of our method through extensive evaluations on circuit problems from the ISCAS-89 and ITC'99 benchmark suites.

==> 06_ablation_study.tex <==
\section{}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> table2.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c} 
\hline
\midrule
SAT  & \# Primary & \# Primary  & \# Variables & \# Clauses & \multicolumn{4}{c}{Throughput (\# Unique Solutions per Second )}\\ 
Instance & Inputs & Outputs & (CNF) &  (CNF) & \textbf{This work} (Speedup) & {\sc UniGen3} & {\sc CMSGen} & {\sc DiffSampler}\\ 
% SAT  & \# Primary & \# Primary  & \# Variables & \# Clauses & \multirow{ 2}{*}{\textbf{This work} (Speedup)} & \multirow{ 2}{*}{{\sc UniGen3}} & \multirow{ 2}{*}{{\sc CMSGen}} & \multirow{ 2}{*}{{\sc DiffSampler}}\\ 
% Instance & Inputs & Outputs & (CNF) &  (CNF) & &  & &\\ 
 \midrule
or-$50$-$10$-$7$-UC-$10$ & $50$ & $4$ & $100$ & $254$ & $\textbf{5,974,780.8}~(79.6\times)$ & $64.7$ & $36,693.5$ & $75,040.1$ \\
% or-$50$-$10$-$7$-UC-$40$ & $50$ & $19$ & $100$ & $250$ & $\textbf{224,660.0}~(5.2\times)$ & $58.3$ & $43,555.0$ & $4,882.8$ \\
%  \midrule
or-$60$-$20$-$10$-UC-$10$ & $60$ & $5$ & $120$ & $305$ & $\textbf{4,777,137.7}~(86.0\times)$ & $81.7$ & $33,987.0$ & $55,521.3$ \\
% or-$60$-$20$-$10$-UC-$40$ & $60$ & $25$ & $120$ & $300$ & $\textbf{2,290,983.7}~(56.5\times)$ & $69.0$ & $40,572.1$ & $7,288.8$ \\
%  \midrule
or-$70$-$5$-$5$-UC-$10$ & $69$ & $7$ & $140$ & $357$ & $\textbf{2,468,613.4}~(77.8\times)$ & $94.5$ & $31,732.4$ & $16,035.1$ \\
% or-$70$-$5$-$5$-UC-$40$ & $69$ & $29$ & $140$ & $350$ & $\textbf{159,326.4}~(3.8\times)$ & $17.4$ & $41,731.9$ & $11,188.1$ \\
%  \midrule
or-$100$-$20$-$8$-UC-$10$ & $98$ & $10$ & $200$ & $510$ & $\textbf{1,707,142.3}~(51.6\times)$ & $43.4$ & $22,951.7$ & $33,175.3$ \\
% or-$100$-$20$-$8$-UC-$60$ & $98$ & $59$ & $200$ & $500$ & $\textbf{354,295.7}~(9\times)$ & $13.6$ & $26,401.4$ & $39,469.4$ \\
 \midrule
$75$-$10$-$1$-q & $83$ & $1$ & $452$ & $443$ & $\textbf{478,723.0}~(42.0\times)$ & $1.6$ & $11,281.8$ & $156.1$ \\
% $75$-$10$-$5$-q & $83$ & $1$ & $460$ & $720$ & $\textbf{1,790,007.7}~(175.1\times)$ & $1.1$ & $10,220.8$ & $373.4$ \\  
$75$-$10$-$10$-q & $79$ & $1$ & $456$ & $439$ & $\textbf{2,075,175.0}~(197.1\times)$ & $1.6$ & $10,527.4$ & $251.8$ \\ 
% \midrule
$90$-$10$-$1$-q & $51$ & $1$ & $432$ & $411$ & $\textbf{2,809,981.5}~(251.7\times)$ & $1.0$ & $11,162.5$ & $227.9$ \\
% $90$-$10$-$5$-q & $45$ & $1$ & $460$ & $720$ & $\textbf{2,644,714.0}~(224.7\times)$ & $2.2$ & $11,771.8$ & $58.5$  \\
$90$-$10$-$10$-q & $31$ & $1$ & $428$ & $391$ & $\textbf{3,567,035.2}~(326.9\times)$ & $1.4$ & $10,913.0$ & $57.9$\\
\midrule
s$15850$a\_$3$\_$2$ & $600$ & $3$ & $10,908$ & $24,476$ & $\textbf{20,267.1}~(47.1\times)$ & $0.4$ & $430.4$ & TO \\
s$15850$a\_$7$\_$4$ & $600$ & $7$ & $10,926$ & $24,552$ & $\textbf{14,930.5}~(34.1\times)$ & $0.5$ & $437.9$ &  TO \\
s$15850$a\_$15$\_$7$ & $600$ & $15$ &  $10,995$ & $24,836$ & $\textbf{14,177.1}~(33.6\times)$ & $0.5$ & $422.2$ & TO \\
\midrule
Prod-$8$  & $293$ & $2$ & $14,952$ & $74,702$ & $\textbf{994.9}~(523.6\times)$ & $1.9$ & $0.2$ & TO \\
Prod-$20$ & $677$ & $2$ & $37,320$ & $186,734$ & $\textbf{139.1}~(347.8\times)$ & $0.4$ & TO &  TO \\
Prod-$32$ & $1061$ & $2$ & $59,688$ & $298,766$ & $\textbf{96.0}~(480\times)$ & $0.2$ & TO &  TO \\
\midrule
\hline
\end{tabular}



